Intrinsic Rewards from Self-Organizing Feature Maps for Exploration in Reinforcement Learning

We introduce an exploration bonus for deep reinforcement learning methods calculated using self-organising feature maps. Our method uses adaptive resonance theory (ART) providing online, unsupervised clustering to quantify the novelty of a state. This heuristic is used to add an intrinsic reward to the extrinsic reward signal for then to optimize the agent to maximize the sum of these two rewards. We find that this method was able to play the game Ordeal at a human level after a comparable number of training epochs to ICM arXiv:1705.05464. Agents augmented with RND arXiv:1810.12894 were unable to achieve the same level of performance in our space of hyperparameters.

==> Lindegaard, Vinje, Severinsen 2022/Sections/0_Abstract.tex <==
\begin{abstract}
We introduce an exploration bonus for deep reinforcement learning methods calculated using self-organising feature maps. Our method uses adaptive resonance theory providing online, unsupervised clustering to quantify the novelty of a state. This heuristic is used to add an intrinsic reward to the extrinsic reward signal for then to optimize the agent to maximize the sum of these two rewards.
%of the agent in addition to the normal extrinsic reward.
We find that this method was able to play the game Ordeal
% optimally
at a human level
after a comparable number of training epochs to ICM \citep{self_supervised_ICM}. Agents augmented with RND \citep{RND_2018} were unable to achieve the same level of performance in our space of hyperparameters.
\end{abstract}

==> Lindegaard, Vinje, Severinsen 2022/Sections/1.5_Related_work.tex <==
\section{Related work}

Previous methods for providing intrinsic reward include use of next-state prediction (\cite{self_supervised_ICM}, \cite{self_supervised_disagreement}) and state recollection \citep{RND_2018}.
The next-state prediction methods derive some exploration bonus $i_t$ from predicting the next state $s_{t+1}$ from the current state and action $(s_t, a_t)$, often through a feature embedding to a lower dimensional space.
The single state recollection methods use the state $s_{t+1}$ alone to assign an exploration bonus $i_t$, intuitively giving some bonus to states dissimilar to what has previously been seen.


% equating to exploration when the given data is the environment state.

Our work centeres around online algorithms of \emph{self-organizing feature maps} for learning structure from data.
Several SOFMs satisfy all the properties required for calculating exploration bonuses.
We consider methods of \emph{adaptive resonance theory} (ART) \citep{grossberg_1976} inspired by computational neuroscience, in particular \emph{Fuzzy ART} \citep{CARPENTER1991759}.

We are using the code base introduced in \citep{curiosity_baseline}, which is a framework for implementing curiosity driven agents in game environments.




==> Lindegaard, Vinje, Severinsen 2022/Sections/1.75_Motivation.tex <==
\section{Motivation}\label{sec:motivation}
Intuitively, the exploration bonuses using next-state prediction and state recollection are in many properties similar to online unsupervised anomaly detection. This is a domain in which ART has shown promising results, being the current state of the art on the Numenta Anomaly Benchmark \citep{ART_2017_anomalydet}.
We suspect this performance translates to giving relevant exploration bonuses for novel states in reinforcement learning.
Therefore, we propose replacing the mechanism for providing exploration bonuses by with SOFMs. Since ART has performed best in class for anomaly detection, we hypothesize it can be used for more sample efficient exploration in game environments. 

As mentioned, SOFMs has all the important functional properties of the exploration bonus in the RL algorithms. These are (a) online learning of data structure, (b) being self-/unsupervised and (c) including a measure of how different the given input is from previously seen data.
This final measure (c) is used as a reward for sampling data differing significantly from previous samples.
This is the heuristic rewarding exploration into previously unseen states.


Intrinsic motivation has been crucial in solving complex RL tasks in exploration heavy environments \citep{RND_2018}, and improving the methods for exploration bonus will allow solving an even wider array of tasks in reinforcement learning. Alternative approaches to the previously explored methods could provide new insight into the reasons for the success and failures of exploration bonus based methods.

% Our project will (1) implement the full method described in \cite{RND_2018}, and (2) implement the described SOFM methods in place of RND and evaluate their relative performance.
% 
% We hypothesize that the use of SOFMs yields similar or improved results compared to RND.
% Additionally, many SOFMs offer better interpretability than the neural networks on which RND is based.
% In conclusion, we intend to contribute with improved interpretability of the mechanism implementing the intrinsic motivation and reward by the use of SOFMs.
% 
% To evaluate the performance of the methods we will use a standard suite of several Atari games \citep{atari_learning2013} and in particular "Montezuma's Revenge".
% The game is considered particularly difficult for RL agents with its extremely sparse rewards and exploration being key to achieving success.
% % Other relevant environments in the same Atari suite are: Freeway, Gravitar, Pitfall!, Private Eye, Solaris, and Venture.
% Evaluation will be done using three different reward schemes: Only extrinsic rewards, only intrinsic rewards, and combining the two.

==> Lindegaard, Vinje, Severinsen 2022/Sections/1_Introduction.tex <==
\section{Introduction}


A central challenge in reinforcement learning (RL) is the tradeoff between exploration and exploitation.
Often times, the reward function, which will ultimately be exploited, does not provide any motivation for exploration.
Lacking motivation to explore, RL agents are often prone to getting stuck in local minima.

The exploration problem is particularly prevalent in environments with sparse rewards, complex state representations, or requiring complicated high-level decisions consisting of several actions concatenated through time.
The use of \emph{intrinsic motivation}, shown to remedy some of these problems \citep{survey_2019}, assigns rewards to actions which by some heuristic explore the environment. With exploration bonuses the policy is still optimized to maximize rewards.
This allows implementation of exploration bonuses by simple modifications to nothing but the reward signal. In this paper, we explore a method of calculating intrinsic reward using a form of online \textit{self-organizing feature maps} (SOFMs).

Our implementation is available at 
\href{https://github.com/mariuslindegaard/curiosity_baselines}{https://github.com/mariuslindegaard/curiosity\_baselines}.


==> Lindegaard, Vinje, Severinsen 2022/Sections/2_Theory.tex <==
\section{Theoretical background}

The following section will give a brief introduction to the overall problem of learning that we seek to solve in reinforcement learning. Then, the \emph{Proximal Policy Optimization (PPO)} algorithm that is used for policy optimization. Lastly, the self-organizing feature map methods ART are introduced, together with how intrinsic rewards are computed.

\subsection{Reinforcement learning algorithms}

% \emph{General overview of the RL problem}


Fundamentally, \emph{reinforcement learning} is about mapping a trajectory or observations to actions in order to maximize a reward signal given by the environment. %\todo{Skal vi fjerne dette sitatet? Er kanskje litt overflødig?}
% This very principle hinges on the \emph{reward hypothesis}, given in \cite{sutton_barto_2020} as


% \begin{adjustwidth}{1cm}{}
% \vspace{0.5cm}
% \textit{That all of what we mean by goals and purposes can be well thought of as the maximization of the expected value of the cumulative sum of a received scalar signal (called reward).}
% \vspace{0.5cm}
% \end{adjustwidth}

Following this, we wish to find a policy that maximizes the discounted expected return, denoted by 
\begin{equation}
    R^{\gamma}(\tau) = \E{\sum_{i=1}^T\gamma^{i-1}r_i(s_i, a_i)}
\end{equation}
where $r_i$ denotes the reward from timestep $i$ by doing action $a_i$ in state $s_i$, $\tau$ denotes the trajectory of the agent and is given as $\tau=\{s_0, a_0, r_0, \dots, s_T, a_T, r_T\}$ and $\gamma\in [0, 1]$ is a given discount factor.

This paper considers \emph{policy gradient methods} where we learn a stochastic policy $\pi_{\theta}(a_t|s_t)$ that defines a probability distribution over actions $a_t$ given the current state $s_t$ parameterized by $\theta\in\mathbb{R}^m$. Actions are then chosen by sampling from this distribution.

Theoretically, we can find the optimal policy based on some training set of samples from the environment and then solve the optimization problem
\begin{equation}\label{eq:theory:theta_argmin}
    \theta^* = \argmax_{\theta} J(\theta)
\end{equation}
for a suitable maximization target given by $J(\theta)$.

\subsection{Proximal Policy Optimization}

There are multiple considerations to take to robustly converge to a solution, most notably variance reduction of the estimated gradient that has to be computed. In order to maximize policy improvement we use the sequential optimization objective
\begin{align}
    \theta_{t+1} &= \theta_t + \Delta \theta_t, \label{eq:policy_improvement_optimize} \\
    \Delta \theta_t &= \argmax_d J(\theta_t+d) - J(\theta_t),
\end{align}
where $d$ denotes a change to the parameters from one iteration to the next. It can be shown \citep{kakade_langford_2002} that the objective can be rewritten as
\begin{align}
    J(\theta + d) - J(\theta) &= \mathbb{E}_{\tau\sim\pi_{\theta + d}}\left[\sum_{t=1}^T\gamma^{t-1}A^{\pi_{\theta}}(s_t, a_t)\right] \\
    &= \mathbb{E}_{\substack{s\sim\pi_{\theta + d}, \\ a\sim\pi_{\theta}}}\left[\frac{\pi_{\theta+d}(a|s)}{\pi_{\theta}(a|s)}A^{\pi_{\theta}}(s,a)\right].\label{eq:objective_J}
\end{align}
where the \emph{advantage}
\begin{equation}
    A^{\pi_{\theta}}(s_t, a_t) = R^{\gamma}(\tau_{t:T}) - b(s_t)
\end{equation}
and where $\tau_{t:T}$ denotes the subtrajectory of the total trajectory only considering the timesteps from $t$ to $T$ and $b(s_t)$ is some bias term dependent on the state $s_t$.

In addition to optimizing the objective in \eqref{eq:objective_J}, it is common to constrain the KL-divergence between the two policies $\pi_{\theta + d}$ and $\pi_{\theta}$. 
Simplifying the KL-convergence constraint, \emph{Proximal Policy Optimization} (PPO) replaces the KL-divergence constraint with a clipping of the ratio $\frac{\pi_{\theta+d}(a|s)}{\pi_{\theta}(a|s)}$ between $1-\epsilon$ and $1 + \epsilon$ for some $\epsilon$ to penalize big changes between the two policies. Thus, the final objective takes the form
\begin{equation}
    J(\theta + d) - J(\theta) = \mathbb{E}_{\substack{s\sim\pi_{\theta + d}, \\ a\sim\pi_{\theta}}}\left[\min\left\{\frac{\pi_{\theta+d}(a|s)}{\pi_{\theta}(a|s)}A^{\pi_{\theta}}(s,a), \mathrm{clip}\left(\frac{\pi_{\theta+d}(a|s)}{\pi_{\theta}(a|s)}, 1-\epsilon, 1+
    \epsilon\right)A^{\pi_{\theta}}(s,a)\right\}\right].
\end{equation}

We will in our experiments be using PPO as the underlying algorithm and let the reward $r_t = e_t \to r_t = e_t + i_t$ where $e_t$ are the extrinsic rewards provided by the environment and $i_t$ are exploration bonuses generated by observing the current state and action. Our experiments will revolve around implementing and evaluating two new methods for providing exploration bonuses $i_t$.

\subsection{Exploration bonuses} \label{sec:Exploration bonuses}

The use of exploration bonuses in RL methods is intuitively meant to encourage exploration even when the extrinsic reward $e_t$ is sparse in the environment.
The agent $\pi$ is trained to maximize the total reward $r_t = e_t + i_t$ where the \emph{intrinsic reward} $i_t$ is some exploration bonus.
Using this exploration bonus the agents can learn tasks in environments with sparser rewards than methods based purely on extrinsic rewards.

There are several methods for assigning exploration bonuses $i_t$. Recent methods demonstrating success include ICM and RND, which here are also used as baselines. The ICM method computes the exploration bonus by first encoding the states $s_t$ and $s_{t+1}$ as the feaatures $\phi(s_t)$ and $\phi(s_{t+1})$, for then to compute a prediction $\hat{\phi}(s_{t+1})$ of the next state in feature space with $\phi(s_t)$ and action $a_t$. The exploration bonus is then given as the prediction error between the next states in feature space \citep{self_supervised_ICM}. RND uses a prediction network $f_{\theta}(x)$ in conjunction with a fixed, random target network $\hat{f}_{\theta}(x)$ to compute exploration bonuses. When a new observation $x$ is received, it is propagated through both networks, and the error between the two outputs is used as exploration bonus. The prediction network is then trained to give a similar output as the target network \citep{RND_2018}. For a more thorough discussion on exploration bonus based methods, the reader is referred to \citep{Understanding_bonus}.

% The important functional properties of exploration bonus based methods in the RL algorithm are (a) online learning of data structure, (b) being self-/unsupervised and (c) including a measure of how different the given input is from previously seen data.
% This final measure (c) is used as a reward for sampling data differing significantly from previous samples.
% This is the heuristic rewarding exploration into previously unseen states.




% %%%%%%%%% %%%%%%%%% %%%%%%%%% %%%%%%%%%
% \subsection{Kohonen feature maps/ART}\label{subsec:KohonenFMs/ART}

% We propose the use of classical methods of self organising maps to calculate the exploration bonus.
% Specifically we will use the following to generate intrinsic rewards from the state data:
% \begin{itemize}
% % Self-Organized Formation of Topologically Correct Feature Maps"
%     \item Kohonen SOFMs \citep{kohonen_1982}
%     \item Adaptive Resonance Theory \citep{grossberg_1976}, in particular ART2 \citep{carpenter_grossberg_1987}. \todo{Update this with the new method of FuzzyART}.
% \end{itemize}

% Common for the two methods is that they satisfy all the requirements (a-c) described in \ref{sec:Exploration bonuses} and thus can be used to generate the exploration bonuses $i_t$. 

% % We will briefly summarize the relatively simple Kohonen feature map to give an idea of the nature of these unsupervised algorithm, leaving out the details of ART2 for now for brevity.

% %%%%%%%%%
% \subsubsection{Kohonen feature map}

% The Kohonen feature map works by sampling data and updating the weights of the map online from discrete samples in a continuous input space. 
% The output space of nodes required a neighborhood measure. 
% In many cases a 2D-space of output nodes (e.g. a layer of $(25\times25)$ nodes) is used, and closeness measure between two nodes may be the multivarate Gaussian pdf. giving the neighborhood function $h(a, b)\propto \exp(-\frac12\|a-b\|^2/\sigma^2)$ where $a, b = (a_1, a_2), (b_1, b_1)$ are nodes in the output space. 
% This neighborhood measure is used to determine the degree to which neighboring nodes are updated together, giving rise to the property of neighboring nodes in the output space corresponding to similar input space activations.

% More concretely we can write the algorithm as in \cref{alg:KohonenSOFM}, where $w_i$ is the weights of node $i$ (i.e. $W[i]$), \textit{lr} is the learning rate and $h$ is the neighborhood function. Note that \textit{input\_dim} and \textit{output\_dim} can be multi-dimensional. Also note that this algorithm is online, yielding a $W$ for each new data sample before continuing iteration.

% \begin{algorithm}
% \caption{Kohonen Self-organising Feature Map}\label{alg:KohonenSOFM}
% \begin{algorithmic}[1]
% \Procedure{Organise Kohonen Map}{\textit{input\_dim, output\_dim, lr}}
%     \State $W \gets $ randomly initialize matrix of shape (\textit{output\_dim}$\times$\textit{input\_dim}).
%     \While{True}
%         \State $x \gets $ SampleInputData()\Comment{Get next data sample}
%         \State \textit{i} $\gets \argmin_j\|x-w_j\|$\Comment{Find the node with the weights closest to the input}
%         \For{$j \in $ range(\textit{output\_dim})}\Comment{Iterate over all output nodes}
%             \State $w_j \gets w_j + $ \textit{lr}$\cdot h(j, i) (x-w_j)$
%         \EndFor
%         \State \textbf{yield} W\Comment{Give current W, then continue iterating}
%     \EndWhile
% \EndProcedure
% \end{algorithmic}
% \end{algorithm}

\subsection{Adaptive Resonance Theory}

% Originally developed in \cite{carpenter_grossberg_1987}, ART2 performs online unsupervised classification on continuous data. For brevity the mathematical theory is not repeated but can be found in the original paper.

% % or in \todo{reference "How does a Brain Build a Cognitive Code"} for a more comprehensive and intuitive introduction.

% Key to our method is that ART2 works as a classifier expanding its number classes as needed.
% Using the size of weight updates to existing classes, expecting bigger changes for larger within-class differences, as well as whether a new class is added form the backbone of our exploration bonus. 

The field of adaptive resonance theory was first introduced by Stephen Grossberg and Gail Carpenter \citep{grossberg_1976,carpenter_grossberg_1987}, and is proposed as a more biologically consistent theory for how the human brain does learning in a constantly evolving environment \citep{art_survey_2019}. As ART is a SOFM, it benefits from the properties listed in \cref{sec:motivation}. However, the perhaps most useful property of ART compared to other, more traditional neural network models is that it addresses the \emph{stability-plasticity dilemma} \citep{carpenter_grossberg_1987a,grossberg_1980} which is about the balance between designing a system that is able to remember previous experiences (stability) while also being able to make new memories based on novel experiences (plasticity). While ART is able to remember previous experiences and also learn new ones, modern, neural networks are in general not, a phenomena called \emph{catastrophic forgetting} \citep{MCCLOSKEY1989109}.

The following treatment of Fuzzy ART is based on \cite{art_survey_2019}.

% \subsubsection{Overall architecture}

% In general, the ART architecture uses two layers that are called the \emph{feature representation field} $\mathrm{F}_1$ and the \emph{category representation field} $\mathrm{F}_2$. Additionally, an \emph{orienting subsystem} is used to regulate decision-making by inhibiting or allowing categories to resonate with inputs. 

\subsubsection{Fuzzy ART}

The used implementation for testing is the \emph{Fuzzy ART} \cite{CARPENTER1991759}, which generalizes the original ART formulation to accept real-valued features by using operators from fuzzy set theory.

First, an augmentation of the input $\bm{\mathsf{x}}\in[0, 1]^d$ is done to prevent proliferation of categories due to to weight erosion \cite{CARPENTER19971473}. Thus, the new, augmented input $\bm{x}$ takes the form
\begin{equation}
    \bm{x} = \begin{bmatrix}\bm{\mathsf{x}} \\ \bm{1} - \bm{\mathsf{x}}\end{bmatrix},\quad \bm{x} \in [0, 1]^{2d}.
\end{equation}
The long-term memory (LTM) in Fuzzy ART is given by a discrete, finite set of weight vectors 
\begin{equation}\label{eq:fuzzy_and:LTM}
\mathcal{W}=\bigcup_{j\in\mathcal{C}}\{\bm{w}_j\}, 
\end{equation}
where $\mathcal{C}= \{1,\dots,C\}$ is the index set over all $C$ categories stored in the LTM so far and $\bm{w}\in[0, 1]^{2d}$. When a new input is presented to Fuzzy ART, the \emph{activation} $T_j$ of this input is computed for each node $\bm{w}_j$ in the LTM as
\begin{equation}
    T_j = \frac{||\bm{x}\wedge \bm{w}_j||_1}{\alpha + ||\bm{w}_j||_1},\quad\forall j\in\mathcal{C}\label{eq:fuzzy_art:activation},
\end{equation}
where $\fuzzyand{\bm{u}}{\bm{v}}$ denotes the \emph{fuzzy AND} of the two vectors $\bm{u},\bm{v}\in\mathbb{R}^n$ and is defined as the vector of element-wise $\min(\cdot)$ of $\bm{u}$ and $\bm{v}$ such that
\begin{equation}
    \fuzzyand{\bm{u}}{\bm{v}} = \brackets{\min(u_1, v_1) \\ \vdots \\ \min(u_n, v_n)},
\end{equation}
the 1-norm $||\bm{u}||_1$ for $\bm{u}\in\mathbb{R}^n$ is
\begin{equation}
    ||\bm{u}||_1 = \sum_{i=1}^n |u_i|,
\end{equation}
and $\alpha>0$ is a regularizing hyperparameter that penalizes large weights. For the next step, define the ordered, sorted index set
% \begin{equation}
$\mathcal{C}^* = \{J~|~J\in\mathcal{C},~T_{J-1} \geq T_J \geq T_{J+1}\}$,
% \end{equation}
\ie, with indices in order of highest activation to lowest. The \emph{vigilance test} is conducted to check for resonance in each node from the input by computing the \emph{vigilance}
\begin{equation}\label{eq:fuzzy_and:vigilance}
    M_J = \frac{||\bm{x}\wedge \bm{w}_J||_1}{||\bm{x}||_1},\quad \forall J\in\mathcal{C}^*  
\end{equation}
and then comparing it to the \emph{vigilance threshold} $\rho\in[0, 1]$
\begin{equation}\label{eq:fuzzy_art:vigiliance_thresh}
    M_J \geq \rho
\end{equation}
where the winning node is the first node $J$ to satisfy \cref{eq:fuzzy_art:vigiliance_thresh}. In case no node satisfy \cref{eq:fuzzy_art:vigiliance_thresh}, a new category is initialized with all weights equal to $1$, such that
\begin{align}
    \bm{w}_{C+1} &= \bm{1}, \\
    \mathcal{W} &\gets \mathcal{W}\cup\{\bm{w}_{C+1}\}, \\
    J &= C + 1.
\end{align}

The last step to Fuzzy ART is the learning step, where the weight $\bm{w}_{J}$ of the winning node $J$ is updated according to
\begin{equation}\label{eq:fuzzy_art:learning}
    \bm{w}_J \gets (1 - \beta)\bm{w}_J + \beta(\fuzzyand{\bm{x}}{\bm{w}_J})
\end{equation}
where $\beta$ is the learning rate. The full algorithm for joint learning and classification of one feature $\bm{x}$ can be found in \cref{alg:FuzzyART}. 

\begin{algorithm}
\caption{Fuzzy ART learning and classification.}\label{alg:FuzzyART}
\begin{algorithmic}[1]
\Procedure{FuzzyART}{$\bm{x}$, $\mathcal{W}$}
    \State $\bm{T}$ $\gets \left[T_j\text{ for }j\text{ in }\mathcal{C}\right]$ \Comment{Compute activation of each node for input with \cref{eq:fuzzy_art:activation}}
    \State $J_{\mathrm{winner}} \gets C + 1$
    \State $\mathcal{C}^* \gets \textsc{SortedSet}(\mathcal{C}, \bm{T})$
    \For{$J\in\mathcal{C}^*$}\Comment{Loop over ordered indices}
        \If{$M_J\geq\rho$} \Comment{Vigilance test based on \cref{eq:fuzzy_and:vigilance} and \cref{eq:fuzzy_art:vigiliance_thresh}}
            \State $J_{\mathrm{winner}}\gets J$
            \State \textbf{break}
        \EndIf
    \EndFor
    \If{$J_{\mathrm{winner}} = C + 1$} \Comment{No node resonated with input, initialize new category}
    \State $\bm{w}_{C+1} \gets \bm{1}$
    \State $\mathcal{W} \gets \mathcal{W}\cup\{\bm{w}_{C+1}\}$
    \EndIf
    \State $\bm{w}_{J_\mathrm{winner}} \gets (1 - \beta)\bm{w}_{J_\mathrm{winner}} + \beta(\fuzzyand{\bm{x}}{\bm{w}_{J_\mathrm{winner}}})$ \Comment{Learning}
    \State \Return $J_{\mathrm{winner}}$
\EndProcedure
\end{algorithmic}
\end{algorithm}


% \begin{algorithm}
% \caption{Fuzzy ART training.}\label{alg:FuzzyART}
% \begin{algorithmic}[1]
% \Procedure{FuzzyART}{$\bm{x}$, \texttt{LTM} from previous call}
%     \State \texttt{activations} $\gets \left[\displaystyle\frac{||\bm{x}\wedge \bm{w}_j||_1}{\alpha + ||\bm{w}_j||_1}\text{for }\bm{w}_j\text{ in \texttt{LTM}}\right]$ \Comment{Compute activation of each node for input}
%     \State \texttt{winner} $\gets $ \texttt{num\_categories}$+1$
%     \For{\texttt{match\_attempt} \textbf{in} \texttt{num\_categories}}
%         \State $J$ $\gets$ \textsc{ArgMax}(\texttt{activations})
%         \State $M_J \gets \displaystyle\frac{||\bm{x}\wedge \bm{w}_j||_1}{||\bm{x}||_1}$
%         \If{$M_J\geq\rho$} \Comment{Vigilance test}
%             \State \texttt{winner} $\gets J$
%             \State \textbf{break}
%         \Else
%             \State \texttt{activations}[$J$] $\gets0$ \Comment{Inhibit the node}
%         \EndIf
%     \EndFor
%     \If{\texttt{winner} $=$ \texttt{num\_categories}$+1$}
%         \State \texttt{LTM} $\gets$ \textsc{AddCategory}(\texttt{LTM}) \Comment{No category resonated with feature, initialize new node}
%         \State \texttt{LTM}[\texttt{winner}] $\gets$ all $1$s
%     \EndIf
%     \State \texttt{LTM}[\texttt{winner}] $\gets\beta(\bm{x}\wedge \bm{w}_{\texttt{winner}}) + (1 - \beta)\bm{w}_{\texttt{winner}}$
%     \State \Return \texttt{winner}
% \EndProcedure
% \end{algorithmic}
% \end{algorithm}

\subsubsection{Batch learning and classification in Fuzzy ART}
% One benefit of using Fuzzy ART as curiosity model is that it is able to ``learn arbitrary input patterns in a fast and stable self-organizing fashion without suffering from catastrophic failure'' \citep{art_survey_2019}, and so using it online can be done in an incremental and unsupervised fashion
In practice, training in Fuzzy ART is done on batches of features $\mathsf{X}=\{\bm{\mathsf{x}}_1, \dots, \bm{\mathsf{x}}_B\}$ simultaneously, which requires a slight modification of the algorithm described in \cref{alg:FuzzyART}. In this case, we do a shuffling of the features in the batch and do learning on all of them sequentially, updating the LTM $\mathcal{W}$ for each, and continuing until the weights $\bm{w}$ of the LTM converges or the number of epochs of training $n_{\mathrm{epoch}}$ surpasses a predetermined threshold $N_{\max}$. See \cref{alg:OnlineBatchFuzzyART} for steps on how to do learning of batches of features.

\begin{algorithm}[H]
\caption{Fuzzy ART for online batch learning. The full \textsc{FuzzyART} learning algorithm can be found in \cref{alg:FuzzyART}.}\label{alg:OnlineBatchFuzzyART}
\begin{algorithmic}[1]
\Procedure{OnlineBatchFuzzyART}{$\mathsf{X}$, $\mathcal{W}$}
    \State $n_{\mathrm{epoch}}\gets 0$
    \While{\textsc{NotConverged}($\mathcal{W}$) \textbf{ and } $n_{\mathrm{epoch}}<N_{\max}$}
        \State $\mathcal{J} \gets \emptyset$ \Comment{Initilize set of classifications by Fuzzy ART on features}
        \State $\mathcal{X}\gets$\textsc{Shuffle}($\mathsf{X}$)
        \For{$\bm{\mathsf{x}}\in\mathcal{X}$}
            \State $\bm{x}$ $\gets \brackets{\bm{\mathsf{x}}\tran & \bm{1}-\bm{\mathsf{x}}\tran}\tran$
            \State $J\gets$\textsc{FuzzyART}($\bm{x}, \mathcal{W}$)
            \State $\mathcal{J}\gets \mathcal{J}\cup \{J\}$ 
        \EndFor
        \State $n_{\mathrm{epoch}}\gets n_{\mathrm{epoch}}+1$
    \EndWhile
    \State \Return $\mathcal{J}$
\EndProcedure
\end{algorithmic}
\end{algorithm}

\subsubsection{Fuzzy ART input encoding}% \todo{Er dette et bra navn på denne section?}

There are two particular practical considerations to make when encoding features to be used by Fuzzy ART.
% In practice, running the Fuzzy ART algorithm takes some consideration.\todo{Dårlig setning?}
Firstly, Fuzzy ART only accepts inputs $\bm{x}\in[0, 1]^d$, and a transformation to perform such a mapping is needed in case this is not the case. Additionally, the observation space might be large, and hence it can be beneficial to represent the features with a more compact encoding for performance reasons. In the experiments, a static feature encoding \emph{head} was used to preprocess the observations for some of the ART models. We also present a \emph{headless} version (ART-HL), working directly on the $(8\times5\times5)$ binary input space of Ordeal.

% As the observation space from Ordeal is of type ``mask'', where the agent observe the presence or absence of each object that exists in the world, and cropped, the observations flattened was only of size $200$ and either $0$ or $1$, and so a \emph{headless} version with no preprocessing of the observations was also used in testing.

% \begin{algorithm}
% \caption{Fuzzy ART for online batch learning. The full \textsc{FuzzyART} learning algorithm can be found in \cref{alg:FuzzyART}.}\label{alg:OnlineBatchFuzzyART}
% \begin{algorithmic}[1]
% \Procedure{OnlineFuzzyART}{\texttt{feature\_batch}, \texttt{LTM} from previous call}
%     \State \texttt{cluster\_choices} $ \gets $ batch size list of zeros
%     \State \texttt{indices} $ \gets $ list of indices over all features in batch
%     \State \texttt{num\_epochs} $\gets 0$
%     \While{\textsc{NotConverged}(\texttt{LTM}) \textbf{and} \texttt{num\_epochs} $<$ \textsc{MaxEpochs}}
%         \State \texttt{shuffled\_indices} $\gets$\textsc{Shuffle}(\texttt{indices})
%         \For{\texttt{index} \textbf{in} \texttt{shuffled\_indices}}
%             \State $\bm{\mathsf{x}} \gets $ \texttt{feature\_batch}[\texttt{index}]
%             \State $\bm{x}$ $\gets [\bm{\mathsf{x}}\quad1-\bm{\mathsf{x}}]$
%             \State \texttt{cluster\_choices}[\texttt{index}] $\gets$ \textsc{FuzzyART}($\bm{x}$, \texttt{LTM})
%         \EndFor
%         \State \texttt{num\_epochs} $\gets$ \texttt{num\_epochs}$+1$
%     \EndWhile
% \EndProcedure
% \end{algorithmic}
% \end{algorithm}


\subsection{Exploration bonus specification}

As discussed, ART will be used as a curiosity model, and so a suitable function for computing the intrinsic reward $i_t$ from an observation $\bm{x}_t$ is necessary. In \cite{Bellemare_2016}, it is argued that a suitable metric for quantifying novelty in the observation is the \emph{information gain} \cite{cover_thomas_1991}, defined as the KL divergence of the \emph{prior state distribution} $\rho_t(x)$, \ie the distribution over $\bm{x}$ prior to an observation $\bm{x}_t$, from its corresponding \emph{posterior distribution} $\rho'(\bm{x})$.
% , which can be computed as
% \begin{equation}
%     \mathrm{KL}(\rho'(\bm{x})~||~\rho(\bm{x})) = \int \rho'(\bm{x})\cdot\log\left(\frac{\rho'(\bm{x})}{\rho(\bm{x})}\right)\mathrm{d}\bm{x}
% \end{equation}
In general, this quantity is often not tractable to compute. They claim, however, that the \emph{prediction gain} $PG_n$, given by $PG_t = \log\rho'_n(\bm{x}_t) - \log\rho_n(\bm{x}_t)$, is a good approximation. They then show that the inverse square-root of the \emph{pseudo-count} $\hat{N}_t(\bm{x})$ over times that state $\bm{x}$ has been visited can be used as an upper bound for the prediction gain as $PG_t \leq \hat{N}_t(\bm{x})^{-1/2}$ in which Bellemare et al. claim that an exploration bonus proportional to $\hat{N}_t(\bm{x})^{-1/2}$ will give behavior that is at least as exploratory as as an exploration bonus based on information gain. 

By denoting Fuzzy ART by the function $j = f(\bm{x})$, where $j$ is the classification of $\bm{x}$ as computed by Fuzzy ART, and introducing the \emph{category count function} $N(j)$, which returns the number of times a category $j$ has been seen by ART, a natural choice for computing the intrinsic reward $i$ is then
\begin{equation}
    i_t(\bm{x}_t) = \frac{k}{\sqrt{N(f(\bm{x}_t))}} \quad k>0
\end{equation}
for an observation $\bm{x}_t$, which is used in the experiments that follow.
 
% The obvious way to determine exploration bonuses from the Kohonen feature map and ART2 algorithm is to measure the total magnitude of weight updates caused by the presented data (i.e. state $s_t$). This heuristic will reflect that unusual points will cause a larger weight update than what the feature maps have already seen, giving a higher exploration bonus to uncommon points.


% One point of caution using these methods is that the subtraction of a baseline might be required as the exploration bonus always will be positive, mirroring the use of the advantage in PPO.
% Scaling of the exploration bonus when training with both the intrinsic and extrinsic rewards might also be an important hyperparameter as we need to ensure the intrinsic rewards are significant but do not dwarf the underlying reward signal.
% Notably, these problems are common for several exploration bonus methods. 

% The major disadvantage of this method is that it might require subtracting the expected value of especially in the case of the Kohonen feature map


% \subsubsection{Evaluation of "outliers" from Khohnen/ART}

% \emph{Key problem: How to make sure we actually get "novel" unpredictable states, not just unpredictable or uncommon (but unexiting, e.g. losing the game) states.}

% \emph{Key principle of ART: No catastrophic forgetting.}



==> Lindegaard, Vinje, Severinsen 2022/Sections/3_Experiments.tex <==
\section{Experiments and results}

The following section will present the experimental setup and environment used to train and test the agents, together with a discussion on the results.

\subsection{Experimental setup}
To test the performance of our proposed methods we have been training our agents using Deepmind's \textit{Pycolab game engine}
\footnote{\href{https://github.com/deepmind/pycolab}{https://github.com/deepmind/pycolab}}
for evaluating the performance of our methods. The specific game we have used is called Ordeal and can be seen in \cref{fig:ordeal}. The goal of the game is to move to a cave to pick up the sword, which gives you one point. Then you should go back to another cave with a duck that approaches you and when you make contact, you kill it and get another point. However, if you did not pick up the sword first, the duck kills you and you get -1 point. The possible outcomes of the games are therefore as seen in \cref{tab:ordeal}
\begin{multicols}{2}
\hspace{0pt}
\vfill
\begin{table}[H]
    \centering
    \begin{tabular}{c|c}
    \toprule
        Game play & Points \\ \hline
        Go straight to room with duck & -1 \\
        Do nothing & 0 \\
        Find sword but not duck & 1 \\
        Find sword then duck & 2 \\
         \bottomrule
    \end{tabular}
    \caption{Outcomes in Ordeal}
    \label{tab:ordeal}
\end{table}
\vfill
\hspace{0pt}
\begin{figure}[H]
    \centering
    \includegraphics[height = 50mm]{figs/game_ordeal.png}
    \includegraphics[height = 50mm]{figs/game_ordeal_sword.png}
    \caption{Visualization of the game environments: Ordeal\newline Left: Starting point. Right: Cave with sword}
    \label{fig:ordeal}
\end{figure}
\end{multicols}


The fact that the agent needs to go into a specific room to get something, before entering a second room is similar to the Atari game Montezuma's revenge. That game was solved with intrinsic reward from RND \citep{RND_2018} but not by traditional DQN \citep{Mnih2015HumanlevelCT}. The similarity is why we wanted to use Ordeal as test our intrinsic reward method, as we would test for similar concepts, but in a simpler environment.




As a success criterion we will use the total extrinsic rewards on this game, compared to other methods for giving exploration bonuses for RL agents.

The state space is the information seen on the screen around the agent. Specifically this is a $(8\times5\times5)$ one hot encoding for each of the 8 types of squares that can appear on screen. The action space is simply moving up, down, left and right, in addition to being able to quit the game.



\subsection{Quantitative results}

Using the different methods for generating intrinsic rewards, we simulate several runs on Ordeal evaluating the average episodic intrinsic rewards. Our results are presented in \cref{fig:performance1}.
The figure shows that after 400k iterations, that ICM is able to converge to the solution in all cases. This makes it the best performing method. The headless ART is able to converge to the optima in some cases, on average achieving a score of around 1. None of the runs with ART with a dimension reducing head or RND for intrinsic reward are able to achieve significant success on the Ordeal environment.

%\vspace{-0.5cm}
\begin{figure}
    \centering
    \includegraphics[height = 60mm]{figs/EpExtrinsicReward.Average.pdf}
    % \includegraphics[height = 50mm]{figs/game_ordeal_sword.png}
    \caption{Performance over training iterations for different intrinsic reward algorithms. The ART-HL method is the headless ART, ART references ART with the static feature encoding head, RND and ICM referencing the methods mentioned in \cref{sec:Exploration bonuses}. The shaded area shows the standard deviation in the results}
    \label{fig:performance1}
\end{figure}
%\vspace{-0.5cm}

As seen by the significant standard deviation on ART-HL and ICM, there is stochasticity in whether the algorithms reach the optimum score after a given set of training episodes.
Continued training appears to increase the probability that convergence occurs for both successful methods, as evidenced by the increasing average score.


\subsection{Qualitative analysis}\label{sec:qualitative_analysis}
From visualizing our agent behaviour through game play, we can see that it goes in a straight line to the room with the sword and then takes what looks like the shortest path to the room with the duck. The agent trained using ART therefore exhibits desired performance at an optimal or close to optimal level. A video of the ART agent solving the game can be found here. \footnote{
\href{https://drive.google.com/drive/folders/1NT1lFBW56kIZcAWlMqHXah3dwfOmHeYn?usp=sharing}{https://drive.google.com/drive/folders/1NT1lFBW56kIZcAWlMqHXah3dwfOmHeYn?usp=sharing}
}

\begin{figure}
    \centering
    \includegraphics[height =80mm]{figs/selected_runs_wide.pdf}
    \caption{Performance over training iterations for different individual agents. The labelling is as in figure \ref{fig:performance1}, with lowercase and index indicating that these are individual agent runs.}
    \label{fig:performance}
\end{figure}

In \cref{fig:performance}, we can see that while RND is the first agent to get one point, it never solves the whole game to achieve 2 points.
The first agent to do this is ART. The intrinsic reward can be seen as the orange line in the second graph. We can see some desired behavior, like the fact that when the agent consistently finds the sword, and therefore moves up to one point in extrinsic reward, it coincides with a spike in the intrinsic reward. This shows a correlation between finding a new room and intrinsic reward. 
However, the jump from one to two, where it learns to go to the duck afterwards, is not associated with the same spike, so is not "rewarded" intrinsically. This might be because the second room is to similar to the first one.

For these typical runs we note the difference in average intrinsic rewards for the different methods.
While all agens have comparable variance in intrinsic reward, RND seems to have a particularly high average intrinsic reward. We hypothesise that this contributes to the fact that this method never converges toward the two-point extrinsic reward optimum, as the PPO agent rather optimizes based on gaining more intrinsic reward and choosing not to end the game.
In numbers, the problem lies in that for the maximal $500$ steps per episode  (See figure \ref{fig:rnd_performance} in Appendix \ref{app:rnd_performance}) and average intrinsic reward hovering around $0.005$ the total intrinsic reward is around $2.5$, greater than the maximal extrinsic reward of $2$. The goals of ending the episode early by finding the sword to kill the duck versus continuing to gain intrinsic reward through a long episode results in, in the case of RND, continuing "exploration" for as long as possible.

Note also the extreme instability in average intrinsic reward for the \verb|art_9| run. This is due to new classes sporadically being created with all samples fitting in this new class having an increased intrinsic reward compared to the other states. Reducing this noise by eventually capping the number of classes is likely one of the main reasons the head-less ART method performs better than the standard ART, as capping the number of classes in this relatively small environment avoids the problem of the intrinsic reward becoming the optimizing target for the PPO agent.

Finally we mention that the agents with no intrinsic reward generally exhibited very little interesting behavior and were therefore left out for brevity and clarity. Nearly all standard agents were unable to achieve any reward signal from the environment, resulting in little to no learning.
This problem is exacerbated by the "quit" option being part of the agent action space, resulting in the agent often quitting early and not exploring the environment.




==> Lindegaard, Vinje, Severinsen 2022/Sections/4_Conclusions.tex <==
\section{Conclusions}

%We have demonstrated the ability of ART to function as an intrinsic reward in reinforcement learning.
Using the sparse reward environment Ordeal we have evaluated several methods for assigning intrinsic rewards to promote exploration of the state space. 
Our results demonstrate the ability of ART to be used as a foundation for calculation exploration bonuses by online state clustering and counting.

While not all algorithms were able to demonstrate convergence to an optimal policy for extrinsic reward, we propose that this might be due to a problem of tuning the intrinsic vs. the extrinsic reward. We leave to future work to explore tuning this parameter further for all methods (ART, ICM \& RND based), as well as the possibility of introducing artificial decay in the intrinsic reward.

Furthermore, the robustness of this method should be evaluated by comparing it to the other approaches in more complex environments with different state spaces and reward structures.

% \cite{Mnih2015HumanlevelCT}

% We have shown that ART has the potential to be used as a method for calculating an exploration bonus. This is because it was able to solve the game environment with sparce reward that DQN without intrinsic reward was not able to find.


==> Lindegaard, Vinje, Severinsen 2022/Sections/8_Ack+Ref.tex <==


% \begin{ack}
% \end{ack}
\section*{Acknowledgments}
We wish to thank to Prof. Pulkit Agrawal and of the 6.484 teaching staff for teaching an inspiring and practical course as well as their guidance and support through the project process.
% \bibliography{references}

% \section*{Contributions}
% All authors contributed to all parts of the project and in equal proportions.

==> Lindegaard, Vinje, Severinsen 2022/Sections/99_Checklist.tex <==

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\section*{Checklist}

%%% BEGIN INSTRUCTIONS %%%
The checklist follows the references.  Please
read the checklist guidelines carefully for information on how to answer these
questions.  For each question, change the default \answerTODO{} to \answerYes{},
\answerNo{}, or \answerNA{}.  You are strongly encouraged to include a {\bf
justification to your answer}, either by referencing the appropriate section of
your paper or providing a brief inline description.  For example:
\begin{itemize}
  \item Did you include the license to the code and datasets? \answerYes{See Section~\ref{gen_inst}.}
  \item Did you include the license to the code and datasets? \answerNo{The code and the data are proprietary.}
  \item Did you include the license to the code and datasets? \answerNA{}
\end{itemize}
Please do not modify the questions and only use the provided macros for your
answers.  Note that the Checklist section does not count towards the page
limit.  In your paper, please delete this instructions block and only keep the
Checklist section heading above along with the questions/answers below.
%%% END INSTRUCTIONS %%%

\begin{enumerate}

\item For all authors...
\begin{enumerate}
  \item Do the main claims made in the abstract and introduction accurately reflect the paper's contributions and scope?
    \answerTODO{}
  \item Did you describe the limitations of your work?
    \answerTODO{}
  \item Did you discuss any potential negative societal impacts of your work?
    \answerTODO{}
  \item Have you read the ethics review guidelines and ensured that your paper conforms to them?
    \answerTODO{}
\end{enumerate}

\item If you are including theoretical results...
\begin{enumerate}
  \item Did you state the full set of assumptions of all theoretical results?
    \answerTODO{}
	\item Did you include complete proofs of all theoretical results?
    \answerTODO{}
\end{enumerate}

\item If you ran experiments...
\begin{enumerate}
  \item Did you include the code, data, and instructions needed to reproduce the main experimental results (either in the supplemental material or as a URL)?
    \answerTODO{}
  \item Did you specify all the training details (e.g., data splits, hyperparameters, how they were chosen)?
    \answerTODO{}
	\item Did you report error bars (e.g., with respect to the random seed after running experiments multiple times)?
    \answerTODO{}
	\item Did you include the total amount of compute and the type of resources used (e.g., type of GPUs, internal cluster, or cloud provider)?
    \answerTODO{}
\end{enumerate}

\item If you are using existing assets (e.g., code, data, models) or curating/releasing new assets...
\begin{enumerate}
  \item If your work uses existing assets, did you cite the creators?
    \answerTODO{}
  \item Did you mention the license of the assets?
    \answerTODO{}
  \item Did you include any new assets either in the supplemental material or as a URL?
    \answerTODO{}
  \item Did you discuss whether and how consent was obtained from people whose data you're using/curating?
    \answerTODO{}
  \item Did you discuss whether the data you are using/curating contains personally identifiable information or offensive content?
    \answerTODO{}
\end{enumerate}

\item If you used crowdsourcing or conducted research with human subjects...
\begin{enumerate}
  \item Did you include the full text of instructions given to participants and screenshots, if applicable?
    \answerTODO{}
  \item Did you describe any potential participant risks, with links to Institutional Review Board (IRB) approvals, if applicable?
    \answerTODO{}
  \item Did you include the estimated hourly wage paid to participants and the total amount spent on participant compensation?
    \answerTODO{}
\end{enumerate}

\end{enumerate}


==> Lindegaard, Vinje, Severinsen 2022/body.tex <==
% \input{body_template}
%\input{Sections/_Abstract proposals}
\input{Sections/0_Abstract}
\input{Sections/1_Introduction}
\input{Sections/1.5_Related_work}
\input{Sections/1.75_Motivation}
\input{Sections/2_Theory}
\input{Sections/3_Experiments}
\input{Sections/4_Conclusions}

\input{Sections/8_Ack+Ref}
\input{Sections/9_Appendix}
% \input{Sections/99 Checklist}

==> Lindegaard, Vinje, Severinsen 2022/body_template.tex <==

\begin{abstract}
  The abstract paragraph should be indented \nicefrac{1}{2}~inch (3~picas) on
  both the left- and right-hand margins. Use 10~point type, with a vertical
  spacing (leading) of 11~points.  The word \textbf{Abstract} must be centered,
  bold, and in point size 12. Two line spaces precede the abstract. The abstract
  must be limited to one paragraph.
\end{abstract}

\section{Submission of papers to NeurIPS 2021}

Please read the instructions below carefully and follow them faithfully.

\subsection{Style}

Papers to be submitted to NeurIPS 2021 must be prepared according to the
instructions presented here. Papers may only be up to {\bf nine} pages long,
including figures. Additional pages \emph{containing only acknowledgments and
references} are allowed. Papers that exceed the page limit will not be
reviewed, or in any other way considered for presentation at the conference.

The margins in 2021 are the same as those in 2007, which allow for $\sim$$15\%$
more words in the paper compared to earlier years.

Authors are required to use the NeurIPS \LaTeX{} style files obtainable at the
NeurIPS website as indicated below. Please make sure you use the current files
and not previous versions. Tweaking the style files may be grounds for
rejection.

\subsection{Retrieval of style files}

The style files for NeurIPS and other conference information are available on
the World Wide Web at
\begin{center}
  \url{http://www.neurips.cc/}
\end{center}
The file \verb+neurips_2021.pdf+ contains these instructions and illustrates the
various formatting requirements your NeurIPS paper must satisfy.

The only supported style file for NeurIPS 2021 is \verb+neurips_2021.sty+,
rewritten for \LaTeXe{}.  \textbf{Previous style files for \LaTeX{} 2.09,
  Microsoft Word, and RTF are no longer supported!}

The \LaTeX{} style file contains three optional arguments: \verb+final+, which
creates a camera-ready copy, \verb+preprint+, which creates a preprint for
submission to, e.g., arXiv, and \verb+nonatbib+, which will not load the
\verb+natbib+ package for you in case of package clash.

\paragraph{Preprint option}
If you wish to post a preprint of your work online, e.g., on arXiv, using the
NeurIPS style, please use the \verb+preprint+ option. This will create a
nonanonymized version of your work with the text ``Preprint. Work in progress.''
in the footer. This version may be distributed as you see fit. Please \textbf{do
  not} use the \verb+final+ option, which should \textbf{only} be used for
papers accepted to NeurIPS.

At submission time, please omit the \verb+final+ and \verb+preprint+
options. This will anonymize your submission and add line numbers to aid
review. Please do \emph{not} refer to these line numbers in your paper as they
will be removed during generation of camera-ready copies.

The file \verb+neurips_2021.tex+ may be used as a ``shell'' for writing your
paper. All you have to do is replace the author, title, abstract, and text of
the paper with your own.

The formatting instructions contained in these style files are summarized in
Sections \ref{gen_inst}, \ref{headings}, and \ref{others} below.

\section{General formatting instructions}
\label{gen_inst}

The text must be confined within a rectangle 5.5~inches (33~picas) wide and
9~inches (54~picas) long. The left margin is 1.5~inch (9~picas).  Use 10~point
type with a vertical spacing (leading) of 11~points.  Times New Roman is the
preferred typeface throughout, and will be selected for you by default.
Paragraphs are separated by \nicefrac{1}{2}~line space (5.5 points), with no
indentation.

The paper title should be 17~point, initial caps/lower case, bold, centered
between two horizontal rules. The top rule should be 4~points thick and the
bottom rule should be 1~point thick. Allow \nicefrac{1}{4}~inch space above and
below the title to rules. All pages should start at 1~inch (6~picas) from the
top of the page.

For the final version, authors' names are set in boldface, and each name is
centered above the corresponding address. The lead author's name is to be listed
first (left-most), and the co-authors' names (if different address) are set to
follow. If there is only one co-author, list both author and co-author side by
side.

Please pay special attention to the instructions in Section \ref{others}
regarding figures, tables, acknowledgments, and references.

\section{Headings: first level}
\label{headings}

All headings should be lower case (except for first word and proper nouns),
flush left, and bold.

First-level headings should be in 12-point type.

\subsection{Headings: second level}

Second-level headings should be in 10-point type.

\subsubsection{Headings: third level}

Third-level headings should be in 10-point type.

\paragraph{Paragraphs}

There is also a \verb+\paragraph+ command available, which sets the heading in
bold, flush left, and inline with the text, with the heading followed by 1\,em
of space.

\section{Citations, figures, tables, references}
\label{others}

These instructions apply to everyone.

\subsection{Citations within the text}

The \verb+natbib+ package will be loaded for you by default.  Citations may be
author/year or numeric, as long as you maintain internal consistency.  As to the
format of the references themselves, any style is acceptable as long as it is
used consistently.

The documentation for \verb+natbib+ may be found at
\begin{center}
  \url{http://mirrors.ctan.org/macros/latex/contrib/natbib/natnotes.pdf}
\end{center}
Of note is the command \verb+\citet+, which produces citations appropriate for
use in inline text.  For example,
\begin{verbatim}
   \citet{hasselmo} investigated\dots
\end{verbatim}
produces
\begin{quote}
  Hasselmo, et al.\ (1995) investigated\dots
\end{quote}

If you wish to load the \verb+natbib+ package with options, you may add the
following before loading the \verb+neurips_2021+ package:
\begin{verbatim}
   \PassOptionsToPackage{options}{natbib}
\end{verbatim}

If \verb+natbib+ clashes with another package you load, you can add the optional
argument \verb+nonatbib+ when loading the style file:
\begin{verbatim}
   \usepackage[nonatbib]{neurips_2021}
\end{verbatim}

As submission is double blind, refer to your own published work in the third
person. That is, use ``In the previous work of Jones et al.\ [4],'' not ``In our
previous work [4].'' If you cite your other papers that are not widely available
(e.g., a journal paper under review), use anonymous author names in the
citation, e.g., an author of the form ``A.\ Anonymous.''

\subsection{Footnotes}

Footnotes should be used sparingly.  If you do require a footnote, indicate
footnotes with a number\footnote{Sample of the first footnote.} in the
text. Place the footnotes at the bottom of the page on which they appear.
Precede the footnote with a horizontal rule of 2~inches (12~picas).

Note that footnotes are properly typeset \emph{after} punctuation
marks.\footnote{As in this example.}

\subsection{Figures}

\begin{figure}
  \centering
  \fbox{\rule[-.5cm]{0cm}{4cm} \rule[-.5cm]{4cm}{0cm}}
  \caption{Sample figure caption.}
\end{figure}

All artwork must be neat, clean, and legible. Lines should be dark enough for
purposes of reproduction. The figure number and caption always appear after the
figure. Place one line space before the figure caption and one line space after
the figure. The figure caption should be lower case (except for first word and
proper nouns); figures are numbered consecutively.

You may use color figures.  However, it is best for the figure captions and the
paper body to be legible if the paper is printed in either black/white or in
color.

\subsection{Tables}

All tables must be centered, neat, clean and legible.  The table number and
title always appear before the table.  See Table~\ref{sample-table}.

Place one line space before the table title, one line space after the
table title, and one line space after the table. The table title must
be lower case (except for first word and proper nouns); tables are
numbered consecutively.

Note that publication-quality tables \emph{do not contain vertical rules.} We
strongly suggest the use of the \verb+booktabs+ package, which allows for
typesetting high-quality, professional tables:
\begin{center}
  \url{https://www.ctan.org/pkg/booktabs}
\end{center}
This package was used to typeset Table~\ref{sample-table}.

\begin{table}
  \caption{Sample table title}
  \label{sample-table}
  \centering
  \begin{tabular}{lll}
    \toprule
    \multicolumn{2}{c}{Part}                   \\
    \cmidrule(r){1-2}
    Name     & Description     & Size ($\mu$m) \\
    \midrule
    Dendrite & Input terminal  & $\sim$100     \\
    Axon     & Output terminal & $\sim$10      \\
    Soma     & Cell body       & up to $10^6$  \\
    \bottomrule
  \end{tabular}
\end{table}

\section{Final instructions}

Do not change any aspects of the formatting parameters in the style files.  In
particular, do not modify the width or length of the rectangle the text should
fit into, and do not change font sizes (except perhaps in the
\textbf{References} section; see below). Please note that pages should be
numbered.

\section{Preparing PDF files}

Please prepare submission files with paper size ``US Letter,'' and not, for
example, ``A4.''

Fonts were the main cause of problems in the past years. Your PDF file must only
contain Type 1 or Embedded TrueType fonts. Here are a few instructions to
achieve this.

\begin{itemize}

\item You should directly generate PDF files using \verb+pdflatex+.

\item You can check which fonts a PDF files uses.  In Acrobat Reader, select the
  menu Files$>$Document Properties$>$Fonts and select Show All Fonts. You can
  also use the program \verb+pdffonts+ which comes with \verb+xpdf+ and is
  available out-of-the-box on most Linux machines.

\item The IEEE has recommendations for generating PDF files whose fonts are also
  acceptable for NeurIPS. Please see
  \url{http://www.emfield.org/icuwb2010/downloads/IEEE-PDF-SpecV32.pdf}

\item \verb+xfig+ "patterned" shapes are implemented with bitmap fonts.  Use
  "solid" shapes instead.

\item The \verb+\bbold+ package almost always uses bitmap fonts.  You should use
  the equivalent AMS Fonts:
\begin{verbatim}
   \usepackage{amsfonts}
\end{verbatim}
followed by, e.g., \verb+\mathbb{R}+, \verb+\mathbb{N}+, or \verb+\mathbb{C}+
for $\mathbb{R}$, $\mathbb{N}$ or $\mathbb{C}$.  You can also use the following
workaround for reals, natural and complex:
\begin{verbatim}
   \newcommand{\RR}{I\!\!R} %real numbers
   \newcommand{\Nat}{I\!\!N} %natural numbers
   \newcommand{\CC}{I\!\!\!\!C} %complex numbers
\end{verbatim}
Note that \verb+amsfonts+ is automatically loaded by the \verb+amssymb+ package.

\end{itemize}

If your file contains type 3 fonts or non embedded TrueType fonts, we will ask
you to fix it.

\subsection{Margins in \LaTeX{}}

Most of the margin problems come from figures positioned by hand using
\verb+\special+ or other commands. We suggest using the command
\verb+\includegraphics+ from the \verb+graphicx+ package. Always specify the
figure width as a multiple of the line width as in the example below:
\begin{verbatim}
   \usepackage[pdftex]{graphicx} ...
   \includegraphics[width=0.8\linewidth]{myfile.pdf}
\end{verbatim}
See Section 4.4 in the graphics bundle documentation
(\url{http://mirrors.ctan.org/macros/latex/required/graphics/grfguide.pdf})

A number of width problems arise when \LaTeX{} cannot properly hyphenate a
line. Please give LaTeX hyphenation hints using the \verb+\-+ command when
necessary.


==> Sections/99_Checklist.tex <==

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\section*{Checklist}

%%% BEGIN INSTRUCTIONS %%%
The checklist follows the references.  Please
read the checklist guidelines carefully for information on how to answer these
questions.  For each question, change the default \answerTODO{} to \answerYes{},
\answerNo{}, or \answerNA{}.  You are strongly encouraged to include a {\bf
justification to your answer}, either by referencing the appropriate section of
your paper or providing a brief inline description.  For example:
\begin{itemize}
  \item Did you include the license to the code and datasets? \answerYes{See Section~\ref{gen_inst}.}
  \item Did you include the license to the code and datasets? \answerNo{The code and the data are proprietary.}
  \item Did you include the license to the code and datasets? \answerNA{}
\end{itemize}
Please do not modify the questions and only use the provided macros for your
answers.  Note that the Checklist section does not count towards the page
limit.  In your paper, please delete this instructions block and only keep the
Checklist section heading above along with the questions/answers below.
%%% END INSTRUCTIONS %%%

\begin{enumerate}

\item For all authors...
\begin{enumerate}
  \item Do the main claims made in the abstract and introduction accurately reflect the paper's contributions and scope?
    \answerTODO{}
  \item Did you describe the limitations of your work?
    \answerTODO{}
  \item Did you discuss any potential negative societal impacts of your work?
    \answerTODO{}
  \item Have you read the ethics review guidelines and ensured that your paper conforms to them?
    \answerTODO{}
\end{enumerate}

\item If you are including theoretical results...
\begin{enumerate}
  \item Did you state the full set of assumptions of all theoretical results?
    \answerTODO{}
	\item Did you include complete proofs of all theoretical results?
    \answerTODO{}
\end{enumerate}

\item If you ran experiments...
\begin{enumerate}
  \item Did you include the code, data, and instructions needed to reproduce the main experimental results (either in the supplemental material or as a URL)?
    \answerTODO{}
  \item Did you specify all the training details (e.g., data splits, hyperparameters, how they were chosen)?
    \answerTODO{}
	\item Did you report error bars (e.g., with respect to the random seed after running experiments multiple times)?
    \answerTODO{}
	\item Did you include the total amount of compute and the type of resources used (e.g., type of GPUs, internal cluster, or cloud provider)?
    \answerTODO{}
\end{enumerate}

\item If you are using existing assets (e.g., code, data, models) or curating/releasing new assets...
\begin{enumerate}
  \item If your work uses existing assets, did you cite the creators?
    \answerTODO{}
  \item Did you mention the license of the assets?
    \answerTODO{}
  \item Did you include any new assets either in the supplemental material or as a URL?
    \answerTODO{}
  \item Did you discuss whether and how consent was obtained from people whose data you're using/curating?
    \answerTODO{}
  \item Did you discuss whether the data you are using/curating contains personally identifiable information or offensive content?
    \answerTODO{}
\end{enumerate}

\item If you used crowdsourcing or conducted research with human subjects...
\begin{enumerate}
  \item Did you include the full text of instructions given to participants and screenshots, if applicable?
    \answerTODO{}
  \item Did you describe any potential participant risks, with links to Institutional Review Board (IRB) approvals, if applicable?
    \answerTODO{}
  \item Did you include the estimated hourly wage paid to participants and the total amount spent on participant compensation?
    \answerTODO{}
\end{enumerate}

\end{enumerate}


==> body_template.tex <==

\begin{abstract}
  The abstract paragraph should be indented \nicefrac{1}{2}~inch (3~picas) on
  both the left- and right-hand margins. Use 10~point type, with a vertical
  spacing (leading) of 11~points.  The word \textbf{Abstract} must be centered,
  bold, and in point size 12. Two line spaces precede the abstract. The abstract
  must be limited to one paragraph.
\end{abstract}

\section{Submission of papers to NeurIPS 2021}

Please read the instructions below carefully and follow them faithfully.

\subsection{Style}

Papers to be submitted to NeurIPS 2021 must be prepared according to the
instructions presented here. Papers may only be up to {\bf nine} pages long,
including figures. Additional pages \emph{containing only acknowledgments and
references} are allowed. Papers that exceed the page limit will not be
reviewed, or in any other way considered for presentation at the conference.

The margins in 2021 are the same as those in 2007, which allow for $\sim$$15\%$
more words in the paper compared to earlier years.

Authors are required to use the NeurIPS \LaTeX{} style files obtainable at the
NeurIPS website as indicated below. Please make sure you use the current files
and not previous versions. Tweaking the style files may be grounds for
rejection.

\subsection{Retrieval of style files}

The style files for NeurIPS and other conference information are available on
the World Wide Web at
\begin{center}
  \url{http://www.neurips.cc/}
\end{center}
The file \verb+neurips_2021.pdf+ contains these instructions and illustrates the
various formatting requirements your NeurIPS paper must satisfy.

The only supported style file for NeurIPS 2021 is \verb+neurips_2021.sty+,
rewritten for \LaTeXe{}.  \textbf{Previous style files for \LaTeX{} 2.09,
  Microsoft Word, and RTF are no longer supported!}

The \LaTeX{} style file contains three optional arguments: \verb+final+, which
creates a camera-ready copy, \verb+preprint+, which creates a preprint for
submission to, e.g., arXiv, and \verb+nonatbib+, which will not load the
\verb+natbib+ package for you in case of package clash.

\paragraph{Preprint option}
If you wish to post a preprint of your work online, e.g., on arXiv, using the
NeurIPS style, please use the \verb+preprint+ option. This will create a
nonanonymized version of your work with the text ``Preprint. Work in progress.''
in the footer. This version may be distributed as you see fit. Please \textbf{do
  not} use the \verb+final+ option, which should \textbf{only} be used for
papers accepted to NeurIPS.

At submission time, please omit the \verb+final+ and \verb+preprint+
options. This will anonymize your submission and add line numbers to aid
review. Please do \emph{not} refer to these line numbers in your paper as they
will be removed during generation of camera-ready copies.

The file \verb+neurips_2021.tex+ may be used as a ``shell'' for writing your
paper. All you have to do is replace the author, title, abstract, and text of
the paper with your own.

The formatting instructions contained in these style files are summarized in
Sections \ref{gen_inst}, \ref{headings}, and \ref{others} below.

\section{General formatting instructions}
\label{gen_inst}

The text must be confined within a rectangle 5.5~inches (33~picas) wide and
9~inches (54~picas) long. The left margin is 1.5~inch (9~picas).  Use 10~point
type with a vertical spacing (leading) of 11~points.  Times New Roman is the
preferred typeface throughout, and will be selected for you by default.
Paragraphs are separated by \nicefrac{1}{2}~line space (5.5 points), with no
indentation.

The paper title should be 17~point, initial caps/lower case, bold, centered
between two horizontal rules. The top rule should be 4~points thick and the
bottom rule should be 1~point thick. Allow \nicefrac{1}{4}~inch space above and
below the title to rules. All pages should start at 1~inch (6~picas) from the
top of the page.

For the final version, authors' names are set in boldface, and each name is
centered above the corresponding address. The lead author's name is to be listed
first (left-most), and the co-authors' names (if different address) are set to
follow. If there is only one co-author, list both author and co-author side by
side.

Please pay special attention to the instructions in Section \ref{others}
regarding figures, tables, acknowledgments, and references.

\section{Headings: first level}
\label{headings}

All headings should be lower case (except for first word and proper nouns),
flush left, and bold.

First-level headings should be in 12-point type.

\subsection{Headings: second level}

Second-level headings should be in 10-point type.

\subsubsection{Headings: third level}

Third-level headings should be in 10-point type.

\paragraph{Paragraphs}

There is also a \verb+\paragraph+ command available, which sets the heading in
bold, flush left, and inline with the text, with the heading followed by 1\,em
of space.

\section{Citations, figures, tables, references}
\label{others}

These instructions apply to everyone.

\subsection{Citations within the text}

The \verb+natbib+ package will be loaded for you by default.  Citations may be
author/year or numeric, as long as you maintain internal consistency.  As to the
format of the references themselves, any style is acceptable as long as it is
used consistently.

The documentation for \verb+natbib+ may be found at
\begin{center}
  \url{http://mirrors.ctan.org/macros/latex/contrib/natbib/natnotes.pdf}
\end{center}
Of note is the command \verb+\citet+, which produces citations appropriate for
use in inline text.  For example,
\begin{verbatim}
   \citet{hasselmo} investigated\dots
\end{verbatim}
produces
\begin{quote}
  Hasselmo, et al.\ (1995) investigated\dots
\end{quote}

If you wish to load the \verb+natbib+ package with options, you may add the
following before loading the \verb+neurips_2021+ package:
\begin{verbatim}
   \PassOptionsToPackage{options}{natbib}
\end{verbatim}

If \verb+natbib+ clashes with another package you load, you can add the optional
argument \verb+nonatbib+ when loading the style file:
\begin{verbatim}
   \usepackage[nonatbib]{neurips_2021}
\end{verbatim}

As submission is double blind, refer to your own published work in the third
person. That is, use ``In the previous work of Jones et al.\ [4],'' not ``In our
previous work [4].'' If you cite your other papers that are not widely available
(e.g., a journal paper under review), use anonymous author names in the
citation, e.g., an author of the form ``A.\ Anonymous.''

\subsection{Footnotes}

Footnotes should be used sparingly.  If you do require a footnote, indicate
footnotes with a number\footnote{Sample of the first footnote.} in the
text. Place the footnotes at the bottom of the page on which they appear.
Precede the footnote with a horizontal rule of 2~inches (12~picas).

Note that footnotes are properly typeset \emph{after} punctuation
marks.\footnote{As in this example.}

\subsection{Figures}

\begin{figure}
  \centering
  \fbox{\rule[-.5cm]{0cm}{4cm} \rule[-.5cm]{4cm}{0cm}}
  \caption{Sample figure caption.}
\end{figure}

All artwork must be neat, clean, and legible. Lines should be dark enough for
purposes of reproduction. The figure number and caption always appear after the
figure. Place one line space before the figure caption and one line space after
the figure. The figure caption should be lower case (except for first word and
proper nouns); figures are numbered consecutively.

You may use color figures.  However, it is best for the figure captions and the
paper body to be legible if the paper is printed in either black/white or in
color.

\subsection{Tables}

All tables must be centered, neat, clean and legible.  The table number and
title always appear before the table.  See Table~\ref{sample-table}.

Place one line space before the table title, one line space after the
table title, and one line space after the table. The table title must
be lower case (except for first word and proper nouns); tables are
numbered consecutively.

Note that publication-quality tables \emph{do not contain vertical rules.} We
strongly suggest the use of the \verb+booktabs+ package, which allows for
typesetting high-quality, professional tables:
\begin{center}
  \url{https://www.ctan.org/pkg/booktabs}
\end{center}
This package was used to typeset Table~\ref{sample-table}.

\begin{table}
  \caption{Sample table title}
  \label{sample-table}
  \centering
  \begin{tabular}{lll}
    \toprule
    \multicolumn{2}{c}{Part}                   \\
    \cmidrule(r){1-2}
    Name     & Description     & Size ($\mu$m) \\
    \midrule
    Dendrite & Input terminal  & $\sim$100     \\
    Axon     & Output terminal & $\sim$10      \\
    Soma     & Cell body       & up to $10^6$  \\
    \bottomrule
  \end{tabular}
\end{table}

\section{Final instructions}

Do not change any aspects of the formatting parameters in the style files.  In
particular, do not modify the width or length of the rectangle the text should
fit into, and do not change font sizes (except perhaps in the
\textbf{References} section; see below). Please note that pages should be
numbered.

\section{Preparing PDF files}

Please prepare submission files with paper size ``US Letter,'' and not, for
example, ``A4.''

Fonts were the main cause of problems in the past years. Your PDF file must only
contain Type 1 or Embedded TrueType fonts. Here are a few instructions to
achieve this.

\begin{itemize}

\item You should directly generate PDF files using \verb+pdflatex+.

\item You can check which fonts a PDF files uses.  In Acrobat Reader, select the
  menu Files$>$Document Properties$>$Fonts and select Show All Fonts. You can
  also use the program \verb+pdffonts+ which comes with \verb+xpdf+ and is
  available out-of-the-box on most Linux machines.

\item The IEEE has recommendations for generating PDF files whose fonts are also
  acceptable for NeurIPS. Please see
  \url{http://www.emfield.org/icuwb2010/downloads/IEEE-PDF-SpecV32.pdf}

\item \verb+xfig+ "patterned" shapes are implemented with bitmap fonts.  Use
  "solid" shapes instead.

\item The \verb+\bbold+ package almost always uses bitmap fonts.  You should use
  the equivalent AMS Fonts:
\begin{verbatim}
   \usepackage{amsfonts}
\end{verbatim}
followed by, e.g., \verb+\mathbb{R}+, \verb+\mathbb{N}+, or \verb+\mathbb{C}+
for $\mathbb{R}$, $\mathbb{N}$ or $\mathbb{C}$.  You can also use the following
workaround for reals, natural and complex:
\begin{verbatim}
   \newcommand{\RR}{I\!\!R} %real numbers
   \newcommand{\Nat}{I\!\!N} %natural numbers
   \newcommand{\CC}{I\!\!\!\!C} %complex numbers
\end{verbatim}
Note that \verb+amsfonts+ is automatically loaded by the \verb+amssymb+ package.

\end{itemize}

If your file contains type 3 fonts or non embedded TrueType fonts, we will ask
you to fix it.

\subsection{Margins in \LaTeX{}}

Most of the margin problems come from figures positioned by hand using
\verb+\special+ or other commands. We suggest using the command
\verb+\includegraphics+ from the \verb+graphicx+ package. Always specify the
figure width as a multiple of the line width as in the example below:
\begin{verbatim}
   \usepackage[pdftex]{graphicx} ...
   \includegraphics[width=0.8\linewidth]{myfile.pdf}
\end{verbatim}
See Section 4.4 in the graphics bundle documentation
(\url{http://mirrors.ctan.org/macros/latex/required/graphics/grfguide.pdf})

A number of width problems arise when \LaTeX{} cannot properly hyphenate a
line. Please give LaTeX hyphenation hints using the \verb+\-+ command when
necessary.

